Modeling the Risk of In-Person Instruction during the COVID-19 Pandemic

During the COVID-19 pandemic, safely implementing in-person indoor instruction was a high priority for universities nationwide. To support this effort at the University, we developed a mathematical model for estimating the risk of SARS-CoV-2 transmission in university classrooms. This model was used to evaluate combinations of feasible interventions for classrooms at the University during the pandemic and optimize the set of interventions that would allow higher occupancy levels, matching the pre-pandemic numbers of in-person courses. Importantly, we determined that requiring masking in dense classrooms with unrestricted seating with more than 90% of students vaccinated was easy to implement, incurred little logistical or financial cost, and allowed classes to be held at full capacity. A retrospective analysis at the end of the semester confirmed the model's assessment that the proposed classroom configuration would be safe. Our framework is generalizable and was used to support reopening decisions at Stanford University. In addition, our framework is flexible and applies to a wide range of indoor settings. It was repurposed for large university events and gatherings and could be used to support planning indoor space use to avoid transmission of infectious diseases across various industries, from secondary schools to movie theaters and restaurants.

==> temp.tex <==

\begin{table}[]
\caption{Comparison of Attack Rate (\%) Between Location of Seats (\cite{sun2020efficacy}, Table 1)}\label{tab:train_data_attack_rates}
\centering
\begin{tabular}{|l|lllllll|}
\hline
\multirow{2}{*}{Rows apart} & \multicolumn{7}{l|}{Columns apart} \\ \cline{2-8} 
 & \multicolumn{1}{l|}{0} & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & \multicolumn{1}{l|}{4} & \multicolumn{1}{l|}{5} & Average \\ \hline
0 & \multicolumn{1}{l|}{…} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}3.53 \\ (2.89–4.31)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}1.65 \\ (1.18–2.31)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.38 \\ (.18–.78)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.38 \\ (.19–.79)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.29\\ (.10–.85)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}1.53 \\ (1.30–1.80)\end{tabular} \\ \hline
1 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.21 \\ (.11–.38)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.24 \\ (.14–.41)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.14 \\ (.06–.32)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.09 \\ (.03–.25)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.03 \\ (.00–.16)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.05 \\ (.00–.30)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}0.14\\ (.10–.20)\end{tabular} \\ \hline
2 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.25 \\ (.14–.45)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.17 \\ (.09–.33)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.23 \\ (.12–.46)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.16 \\ (.07–.36)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.09\\ (.03–.27)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.17 \\ (.06–.50)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}0.18 \\ (.13–.25)\end{tabular} \\ \hline
3 & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.05 \\ (.01–.18)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.05 \\ (.01–.17)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.13 \\ (.05–.33)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.10 \\ (.03–.30)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.10 \\ (.03–.30)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.06 \\ (.00–.36)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}0.08 \\ (.05–.13)\end{tabular} \\ \hline
Average & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.17 \\ (.12–.26)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.68 \\ (.56–.81)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.41 \\ (.31–.54)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.16\\ (.1–.25)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.12 \\ (.07–.20)\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}0.13 \\ (.06–.25)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}0.32 \\ (.28–.36)\end{tabular} \\ \hline
\end{tabular}
\end{table}

